Popularity Bias in Recommendation: A Multi-stakeholder Perspective

Traditionally, especially in academic research in recommender systems, the focus has been solely on the satisfaction of the end-user. While user satisfaction has, indeed, been associated with the success of the business, it is not the only factor. In many recommendation domains, there are other stakeholders whose needs should be taken into account in the recommendation generation and evaluation. In this dissertation, I describe the notion of multi-stakeholder recommendation. In particular, I study one of the most important challenges in recommendation research, popularity bias, from a multi-stakeholder perspective since, as I show later in this dissertation, it impacts different stakeholders in a recommender system. Popularity bias is a well-known phenomenon in recommender systems where popular items are recommended even more frequently than their popularity would warrant, amplifying long-tail effects already present in many recommendation domains. Prior research has examined various approaches for mitigating popularity bias and enhancing the recommendation of long-tail items overall. The effectiveness of these approaches, however, has not been assessed in multi-stakeholder environments. In this dissertation, I study the impact of popularity bias in recommender systems from a multi-stakeholder perspective. In addition, I propose several algorithms each approaching the popularity bias mitigation from a different angle and compare their performances using several metrics with some other state-of-the-art approaches in the literature. I show that, often, the standard evaluation measures of popularity bias mitigation in the literature do not reflect the real picture of an algorithm's performance when it is evaluated from a multi-stakeholder point of view.

==> tables/lastfm_itemknn_results.tex <==
%\captionsetup[table]{skip=4pt}

\begin{table*}[t]

%\small
\centering
%\setlength{\tabcolsep}{3pt}
\captionof{table}{Results of different algorithms on two datasets. The setting that yields the same precision for all three reranking methods XQ, DM and CP is chosen and the results is reported. Bold values are statistically significant compared to the second best value in each column with significance level of 0.05 ($\alpha$=0.05) } 
\label{tab:overall}
\begin{tabular}{lccccccl}
\toprule
           & Agg-Div & Gini &$Gini_g^C$ &$PCal$&$\bar{ESF}$&$PSF$&$Gini_g^S$
           \\\midrule
Base    &0.131  & 0.942&0.905&0.406&3.658&0.535&0.9018\\
XQ & 0.176 &0.917&0.831&0.486&3.834&0.643&0.844\\
KDD & \textbf{0.393} &\textbf{0.713}&0.702 &0.541&3.957&0.722&0.745\\
CP   &0.260 & 0.831 &\textbf{0.620}&\textbf{0.719}&\textbf{4.240}&\textbf{0.791}&\textbf{0.627}\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/movielens_itemknn_results.tex <==
%\captionsetup[table]{skip=4pt}

\begin{table*}[t]

%\small
\centering
%\setlength{\tabcolsep}{3pt}
\captionof{table}{Results of different algorithms on two datasets. The setting that yields the same precision for all three reranking methods XQ, DM and CP is chosen and the results is reported. Bold values are statistically significant compared to the second best value in each column with significance level of 0.05 ($\alpha$=0.05) } 
\label{tab:overall}
\begin{tabular}{lccccccl}
\toprule
           & Agg-Div & Gini &$Gini_g^C$ &$PCal$&$\bar{ESF}$&$PSF$&$Gini_g^S$
           \\\midrule
Base    & 0.029  & 0.950 &0.999& 0.39& 2.349 &0.44&0.9527\\
XQ & 0.107  & 0.888 &0.817&0.515&2.524 &0.632&0.687\\
KDD & \textbf{0.127}  & \textbf{0.734}&0.779 &0.522&2.630  &0.602&0.742\\
CP   & 0.076  & 0.900& \textbf{0.560}& \textbf{0.700}&\textbf{3.110}&\textbf{0.732}&\textbf{0.561}\\
\bottomrule
\end{tabular}
\end{table*}
